Improving Your Graph Neural Networks: A High-Frequency Booster

Graph neural networks (GNNs) hold the promise of learning efficient representations of graph-structured data, and one of its most important applications is semi-supervised node classification. However, in this application, GNN frameworks tend to fail due to the following issues: over-smoothing and heterophily. The most popular GNNs are known to be focused on the message-passing framework, and recent research shows that these GNNs are often bounded by low-pass filters from a signal processing perspective. We thus incorporate high-frequency information into GNNs to alleviate this genetic problem. In this paper, we argue that the complement of the original graph incorporates a high-pass filter and propose Complement Laplacian Regularization (CLAR) for an efficient enhancement of high-frequency components. The experimental results demonstrate that CLAR helps GNNs tackle over-smoothing, improving the expressiveness of heterophilic graphs, which adds up to 3.6% improvement over popular baselines and ensures topological robustness.

==> tab/tab_hyper.tex <==
% \begin{table*}[h]
%     \centering
%     \caption{Hyper-parameter Settings of CLAR for Random Splits}
%     \begin{tabular}{ccccccccc}
%     \toprule
%              &  Learning rate & Dropout & Hidden size & Weight decay & $\alpha$ & $\beta$ & $S$\\
%     \midrule
%     CiteSeer & 0.01 & 0.5 & 64 & 0.0005 & 0.0 & 1.0 & 1 (121,212)\\
%         Cora & 0.01 & 0.5 & 64 & 0.0005 & 2.0 & 1.0 & 1 (101,011)\\
%   Computers & 0.01 & 0.5 & 64 & 0.0005 & 2.0 & 1.0 & 1 (021,012)\\
%       Photo & 0.01 & 0.5 & 64 & 0.0005 & 2.0 & 0.0 & 1 (212,222)\\
%       PubMed & 0.01 & 0.5 & 64 & 0.0000 & 2.0 & 0.0 & 1 (122,012)\\
%       Actor & 0.05 & 0.5 & 64 & 0.0000 & 2.0 & 1.0 & 1 (011,121)\\
%   Chameleon & 0.05 & 0.5 & 64 & 0.0000 & 1.0 & 2.0 & 2 (122,221)\\
%     Squirrel & 0.05 & 0.5 & 64 & 0.0000 & 2.0 & 1.0 & 2 (012,121)\\
%      Cornell & 0.05 & 0.5 & 64 & 0.0005 & 2.0 & 1.0 & 1 (222,011)\\
%       Texas & 0.05 & 0.5 & 64 & 0.0005 & 0.0 & 2.0 & 1 (221,221)\\
%     \bottomrule
%     \end{tabular}
%     \label{tab:hyper}
% \end{table*}
\begin{table*}[ht]
    \centering
    \caption{Hyper-parameter Settings of CLAR for Random Splits}
    \begin{tabular}{ccccccccccccccc}
    \toprule
             &  \multirow{2}{*}{Learning rate} & \multirow{2}{*}{Dropout} & \multirow{2}{*}{Hidden size} & \multirow{2}{*}{Weight decay} & \multicolumn{3}{c}{GCN} & \multicolumn{3}{c}{GAT} & \multicolumn{3}{c}{SAGE} \\
    \cmidrule(r){6-8} \cmidrule(r){9-11} \cmidrule(r){12-14}
             & &&&& $\alpha$ & $\beta$ & $S$ & $\alpha$ & $\beta$ & $S$ & $\alpha$ & $\beta$ & $S$\\
    \midrule
    CiteSeer & 0.01 & 0.5 & 64 & 0.0005 & 0.0 & 1.0 & 1 & 1.0 & 2.0 & 1 & 2.0 & 1.0 & 2\\
        Cora & 0.01 & 0.5 & 64 & 0.0005 & 2.0 & 1.0 & 1 & 1.0 & 0.0 & 1 & 0.0 & 1.0 & 1\\
  Computers & 0.01 & 0.5 & 64 & 0.0005 & 2.0 & 1.0 & 1 & 0.0 & 2.0 & 1 & 0.0 & 1.0 & 2\\
      Photo & 0.01 & 0.5 & 64 & 0.0005 & 2.0 & 0.0 & 1 & 2.0 & 1.0 & 2 & 2.0 & 2.0 & 2\\
      PubMed & 0.01 & 0.5 & 64 & 0.0000 & 2.0 & 0.0 & 1 & 1.0 & 2.0 & 2 & 0.0 & 1.0 & 2\\
      \midrule
      Actor & 0.05 & 0.5 & 64 & 0.0000 & 2.0 & 1.0 & 1 & 0.0 & 1.0 & 1 & 1.0 & 2.0 & 1\\
  Chameleon & 0.05 & 0.5 & 64 & 0.0000 & 1.0 & 2.0 & 2 & 1.0 & 2.0 & 2 & 2.0 & 2.0 & 1\\
    Squirrel & 0.05 & 0.5 & 64 & 0.0000 & 2.0 & 1.0 & 2 & 0.0 & 1.0 & 2 & 1.0 & 2.0 & 1\\
     Cornell & 0.05 & 0.5 & 64 & 0.0005 & 2.0 & 1.0 & 1 & 2.0 & 2.0 & 2 & 0.0 & 1.0 & 1\\
      Texas & 0.05 & 0.5 & 64 & 0.0005 & 0.0 & 2.0 & 1 & 2.0 & 2.0 & 1 & 2.0 & 2.0 & 1\\
    \bottomrule
    \end{tabular}
    \label{tab:hyper}
\end{table*}

==> tab/tab_hyper_ag.tex <==
\begin{table*}[h]
    \centering
    \caption{Hyper-parameter Settings of CLAR for Planetoid Splits}
    \begin{tabular}{cccccccc}
    \toprule
                & Learning rate & Dropout & Hidden size & Weight decay & $\alpha$ & $\beta$ & $S$ \\
    \midrule
        Cora     & 0.01 & 0.5 & 64 & 0.0005 & 0.005    & -0.005  &  2  \\
        CiteSeer & 0.01 & 0.5 & 64 & 0.0005 & 0.005    & 0.005   &  2  \\
        PubMed   & 0.01 & 0.5 & 64 & 0.0000 & -0.001   & 0.001   &  2  \\
        CS       & 0.01 & 0.5 & 64 & 0.0005 & 0.001    & 0.001   &  2  \\
        Physics  & 0.01 & 0.5 & 64 & 0.0005 & 0.005    & 0.001   &  2  \\
    \bottomrule
    \end{tabular}
    \label{tab:hyper_ag}
\end{table*}

==> tex/intro_back_up.tex <==


\section{Introduction}
Graph neural networks (GNNs) is of high practical value in nowadays' research, in which enhances the progress in various domains~\cite{2021GNNs}, e.g., forecasting the publications' classes on citation networks and deciding the proteins' functions based on protein-protein interactions networks. 
% \textcolor{blue}{In particular, semi-supervised node classification~\cite{kipf2016semi} gains more and more attention due to its wide applicability,
% % where semi-supervised node classification is one of the essential tasks~\cite{2021GNNs}, 
% e.g., forecasting the publications' classes on citation networks and deciding the proteins' functions based on protein-protein interactions networks. }
In essence, 
GNNs learn a function (i.e., filter) taking the eigenvalues (i.e., frequency components) obtained from eigendecomposition of the graph Laplacian matrix as arguments \citep{DBLP:conf/icml/WuSZFYW19,DBLP:conf/iclr/BalcilarRHGAH21} from a spectrum perspective. 
To avoid eigendecomposition, 
In early stage, 
polynomial-based spectral filters alternate to approximately utilize the polynomials (e.g., Cheby-GCN~\citep{DBLP:conf/nips/DefferrardBV16}).
%
\citet{DBLP:conf/iclr/KipfW17} simplify the first-order polynomial term and propose GCN, where the connected neighbors aggregate for updating the central nodes.
%
Because it endues the spectral filters with spatial signification, this paradigm formalizes the modern graph neural networks (GNNs).

\begin{figure}[t]
    \centering
    \includegraphics[trim=2.5cm 0cm 1cm 0cm,clip=true,width=0.5\textwidth]{figures/frequency.pdf}
    \caption{We investigate the frequency components on Chameleon and CiteSeer. On the left, we retain 1) $0$ to the current frequency component $\lambda$ (dashed lines), and 2) successive $50$ sorted frequency components (solid lines) to train and evaluate an MLP. For example, the high-frequency part (the red area) shows equal importance to the low-frequency part, especially on Chameleon (heterophily). On the right, we train Cheby-GCN and BernNet with $10$-order; the high-frequency responses are also positively captured, particularly on the heterophily Chameleon (right).\textcolor{red}{less is more, what do you want your readers pay the most attention to...}}
    \label{fig:freq}
\end{figure}

%
% Subsequently GAT~\citep{DBLP:conf/iclr/VelickovicCCRLB18} and SAGE~\citep{DBLP:conf/nips/HamiltonYL17} are important variants for modern GNNs.
% , which lefts the learned filter returning high value from the low-frequency components and really low value from the high-frequency ones, named the low-pass filter. 
However, recent studies prove that GNNs act as a type of Laplacian smoothing, a low-pass filter~\citet{DBLP:conf/aaai/LiHW18}. When reaching out for higher-order neighbors via stacking layers, the GNNs are getting more strictly low-pass, and the connected nodes would converge to similar values, called over-smoothing~\citep{DBLP:conf/icml/ChenWHDL20,DBLP:conf/icml/WuSZFYW19}.
It dissolves the characteristic of each node and leads to poor performance.
%
On the other hand, this feature is suitable for homophily graphs where the neighbors behave resemblance~\citep{kipf_deep_2020}, while defective for heterophily graphs, where the neighbors are disparate~\citep{DBLP:conf/aaai/BoWSS21}.

These facts and drawbacks motivate us to ask: \textit{only the low-frequency components are required?}

We investigate the frequency components for homophily and heterophily graphs. In Figure~\ref{fig:freq}, high-frequency components (the red area) show the capability to classify as the low-frequency components (the left figure), especially on Chameleon, a heterophily graph. Apart from this, Cheby-GCN and adaptive spectral filters, BernNet~\citep{DBLP:journals/corr/abs-2106-10994} also capture the high-frequency components, whereas Chameleon also returns a more significant frequency response. These observations shed light on that high-frequency components are also practical. 
%
%  heterophily, that high-pass filter encourages to differ the neighbors, in line with the character of them.

Then we attempt to figure out, \textit{how to enhance high-frequency components for GNNs?}

In this paper, we start from the spectral view to argue that the complement of the original graph incorporates a high-pass filter and propose Complement LAplacian Regularization (CLAR) to enhance high-frequency components for GNNs.
%
In CLAR, we adopt 1) random sampling strategies to better capture the frequency components on the complement and 2) the original Laplacian regularization to balance the noisy connections from the sampling.
%
Remarkably, our proposal is incomparable to existing regularization methods for enhancing high-frequency components. 


% Moreover, our proposal is an efficient approach to adjust the shape of the filters of GNNs that saves the computational cost of the spectral graph convolutions. 

Our contributions are as follows:

\begin{itemize}
    \item We investigate that the high-frequency components are also effective for graph learning and argue that the complement of the original graph incorporates a high-pass filter of the frequency components.
    \item Based on our argument, we propose a model-agnostic plugin (CLAR) that enhances the high-frequency components for GNNs via regularizing the complement.  
    \item Experiments on homophily and heterophily graphs show CLAR can alleviate over-smoothing, better depict the heterophily graphs, and improve robustness against topological noise.
\end{itemize}
 



==> tex/x_math.tex <==
\section{Mathematical Justifications}
In this section, we present the spectral examination of CLAR and other regularization methods. We argue that our proposal uniquely obtain high-pass filters. 
\label{sec:math}
\subsection{Spectral Examination of CLAR}
Special note here, we separate the optimization problem of feature transformation (e.g., $\mathcal{L}_{sup}$ in Eq.~\ref{equ:semi}) and that of the propagation (e.g., $\mathcal{L}_{reg}$ in Eq.~\ref{equ:semi}). The following discussions are in the context of the propagation objective. On this basis, GNNs are bridged to their spectral explanations. 

Let us first look at the propagation of GCN~\citep{DBLP:conf/iclr/KipfW17} as an example of GNNs, where re-normalization trick with self-loops is utilized. Suppose that $Z^{(l+1)}=\tilde{\hat{A}}Z^{(l)}$, where $Z^{(0)}=X\Theta^*$ and $\Theta^*$ is the optimal parameters of feature transformation (e.g., full-connected layers). GCN optimizes the following regularization objective~\citep{DBLP:conf/www/ZhuWSJ021}, extended to Lemma~\ref{lemma2}. 
\begin{equation}
    \mathcal{L}_{GCN}=\min_{Z} \tr(Z^T\tilde{\hat{L}}Z),
\label{equ:gcn_optim}
\end{equation}
where $\tr(\cdot)$ is calculating the trace of a matrix.

\newtheorem{lemma}{Lemma}
\newtheorem{remark}{Remark}
\newtheorem{claim}{Claim}
\newtheorem{prop}{Proposition}
\begin{lemma}
\label{lemma2}
The explicit optimization problem defined on Laplacian matrix (e.g., Eq.~\ref{equ:gcn_optim}) could be approximated by a layer-wise propagation network building on the corresponding adjacency matrix (e.g., GCN), and vice versa.
\end{lemma}
In Lemma~\ref{lemma2}, the 'corresponding adjacency matrix' in the propagation denotes convolution matrix~\citep{DBLP:conf/iclr/BalcilarRHGAH21}. Besides, we introduce frequency response, a continuous function defined in the space of graph spectrum, e.g, $\Phi(\lambda)$.
Then, the propagation layer and the frequency response could be bridged by \cite{DBLP:conf/iclr/BalcilarRHGAH21}. Still, we take GCN for example, whose convolution matrix is $\tilde{\hat{A}}$. The spectral components (also spectrum) of $\tilde{\hat{L}}$ is $\lambda=\{\lambda_i,i=1,2,\cdots,n\}$. And frequency response of GCN is $\Phi_{GCN}(\lambda_i) \approx 1-\lambda_i$, leading to Lemma~\ref{lemma1}.
\begin{lemma}
\label{lemma1}
For any convolution matrix directly defined on adjacency matrix  $A$, its frequency response $\Phi_{A}$ is negatively linear correlated to the spectrum of Laplacian matrix of $A$. Specifically, $\Phi_{A}(\lambda_i) \approx 1-\lambda_i$ is a low-pass filter.
\end{lemma}
% In Lemma~\ref{lemma1}, the spectral components $\lambda$ usually draw from normalized Laplacian matrix. 
\begin{prop}
\label{prop}
An Laplacian regularization constructed on the complement incorporates the high-pass filters.
\end{prop}
\textbf{Proof.} Suppose a larger edges set $\mathcal{E}^*$, that $\mathcal{E} \cup \mathcal{E}^*$. A sampled complement $\mathcal{E}_s \subset \mathcal{V}\times \mathcal{V}\cap\mathcal{E}$ can be donated by $\mathcal{E}^* \cap \mathcal{E}$ without any loss of generality. 
Then, the corresponding adjacency matrix is $A_s=A^*-A$, and we obtain the Laplacian regularization objective (the same to Eq.~\ref{equ:com}):
\begin{align}
    \mathcal{L}_{com} &= \min_Z \gamma \tr\left(Z^T\tilde{\mathrm{L}}\left(A^*-A\right)Z\right) \\
    &= \min_Z \gamma \left(\tr\left(Z^T\tilde{\mathrm{L}}\left(A^*\right)Z\right)-\tr\left(Z^T\tilde{\hat{L}}Z\right)\right).
    \label{equ:prop}
\end{align}
Omitting the hyper-parameter $\gamma$, $\tr(Z^T\tilde{\hat{L}}Z))$ is equivalent to GNNs with the convolution matrix $\tilde{A}$, using Lemma~\ref{lemma2}. Next, this convolution returns the frequency responses as  $\left(1-\lambda\right)$ approximately, a low-pass filter on $\tilde{\mathrm{L}}(X)$ induced from Lemma~\ref{lemma1}. However, Eq.~\ref{equ:prop} contains a negation on $\tr(Z^T\tilde{\hat{L}}Z))$, that $\Phi_{A}(\lambda)\approx-\left(1-\lambda\right)$. This formulation points out a negation on the low-pass filter incorporates a high-pass one.

Our main claim that CLAR obtains a \textit{high-pass} filter evidenced by Proposition~\ref{prop}. In CLAR, however, the spectrum of $\tilde{\mathrm{L}}(A^*)$ is not ensured due to the random sampling, i.e., $\Phi_{A^*}(\lambda^*)\approx1-\lambda^*$, which is a low-pass filter on $\tilde{\mathrm{L}}(A^*)$. To this, we deploy a low-pass filter on $\tilde{\mathrm{L}}(A)$ (i.e., Eq.~\ref{equ:ori}) to trade-off the unexpected condition.
 
\input{tab_data}
\textbf{Remark.} 
The hyper-parameter $\alpha$ and $\beta$ can appropriately shape the filters. For example, increasing $\alpha$ represents enhancing the low-pass filters behaving the same as Laplacian regularization (i.e., Eq.~\ref{equ:reg}). Similarly, the high frequency components can be enhanced via increasing $\beta$. 
Additionally, since the sampling multiple $S$ is not directly related to $\lambda^*$, it is not sensitive to CLAR, that is consistent with our experiments (Table~\ref{tab:spearman} in Appendix~\ref{app:s}).

\subsection{Comparisons to Other Regularization Methods}
In order to certify that only CLAR obtains a high-pass filter making it superior, we extensively discuss five other regularization methods, including Network Lasso (Laplacian regularization)~\cite{nlasso}, P-reg~\citep{DBLP:conf/aaai/0002MC21}, MADReg~\citep{DBLP:conf/aaai/ChenLLLZS20}, AdaGraph~\citep{DBLP:conf/aaai/ChenLLLZS20} and DropEdge~\citep{DBLP:conf/iclr/RongHXH20}. 
For simplification, we omit the hyper-parameter ahead every regularization methods (e.g., $\gamma$ in Eq.~\ref{equ:semi}).
\subsubsection{Network Lasso~(NL)}
Network Lasso (Eq.~\ref{gl_optim}) \citep{nlasso} is identical to the Laplacian regularization in Eq.~\ref{equ:semi}~\citep{kipf_deep_2020}, a low-pass filter, which is covered in GCN (Eq.~\ref{equ:gcn_optim}) and CLAR(Eq.~\ref{equ:ori}). Therefore, its improvement stays trivial.
\begin{equation}
    \mathcal{L}_{NL}=\min_{Z} \tr(Z^T\tilde{\hat{L}}Z).
\label{gl_optim}
\end{equation}

\subsubsection{P-reg~(P)}
P-reg (Eq.~\ref{p_optim}) is a penalty on the difference of $Z$ and GCN-smoothed $\tilde{\hat{A}}Z$, which is equivalent to squared Laplacian regularization using squared error~\citep{DBLP:conf/aaai/0002MC21}. 
\begin{equation}
    \mathcal{L}_{P}=\min_{Z} \tr(Z^T\tilde{\hat{L}}^T\tilde{\hat{L}}Z).
    \label{p_optim}
\end{equation}
% Since $\tilde{\hat{L}}$ is symmetric, 
The convolution matrix of P-reg is the adjacency matrix of $\tilde{\hat{L}}^2$. According to Lemma~\ref{lemma1}, its frequency response is $\Phi_{P-reg}(\lambda)\approx1-\lambda^2$, as the spectrum component of $\tilde{\hat{L}}^2$ is $\lambda^2$. Therefore, P-reg is still a low-pass filter that holds more low-frequency components compared to NL.
\subsubsection{MADReg~(MR)}
MADreg (Eq.~\ref{mad_optim}) proposes penalty on the difference of the higher-order neighbors and the lower-order neighbors to alleviate over-smoothing. In specific, the $k$-order neighbors are obtained by stacking $k$ layers (e.g., GCN layers). Practically, MADReg take $8\geq$ for the higher-order and $\leq 3$ for the lower-order. 
\begin{equation}
    \mathcal{L}_{MR}=\min_{Z} \tr(Z^T((Q-\tilde{\mathrm{L}}(\tilde{A^7}))-\tilde{\mathrm{L}}(\tilde{A^3}))Z)
    \label{mad_optim}
\end{equation}
$Q$ is a matrix of ones, and $(Q-\tilde{\mathrm{L}}(\tilde{A^7}))$ signifies higher-order neighbors that $k\geq8$. Approximating the Laplacian of the power adjacency matrix to the power of the Laplacian matrix, that $\tilde{\mathrm{L}}(\tilde{A^k})\approx\tilde{\mathrm{L}}(\tilde{A})^k$, separately we have 
\begin{align*}
    \mathcal{L}_{MR}&\approx\min_{Z} \tr(Z^TQZ)
    -\tr(Z^T\tilde{\mathrm{L}}(\tilde{A})^7Z)\\
    &-\tr(Z^T\tilde{\mathrm{L}}(\tilde{A})^3Z).
\end{align*}
Leaving the independent first term, we derive the frequency responses of MADReg, that $-\Phi_{MR}(\lambda)\approx(1-\lambda)^3+(1-\lambda)^7$, which is a negation of two more extreme low-pass filters, that makes the high-frequency components not distinctive.

\subsubsection{AdaGraph~(AG)}
AG (Eq.~\ref{ag_optim}) modifies Network Lasso (Eq.~\ref{gl_optim}) via adding and dropping edges to $A$. \textbf{DropEdge~(DE)} is a special case of AG, when $A_{add}=[0]_{N\times N}$.
\begin{equation}
    \mathcal{R}_{AG}=\min_{Z} \tr(Z^T\tilde{\mathrm{L}}(A-A_{drop}+A_{add})Z)
    \label{ag_optim}
\end{equation}
 Practically, $l1$-norm regularization is constrained on $A_{add}$ and $A_{drop}$, making them sparse~\citep{DBLP:conf/aaai/ChenLLLZS20}. Consequently, the low-pass filter of $\tilde{\mathrm{L}}(A)$ leads the optimization problem.
\input{tab_filter}


==> tex/x_method.tex <==
\section{Methodology}
We first introduce two sampling methods to explore the complement. Then, we illustrate how to utilize and modify Laplacian regularization for building CLAR on GNNs. The overall architecture of CLAR is shown as Fig.\ref{fig:clar}.
\begin{figure*}[t]
    \centering
    \includegraphics[trim=2cm 0cm 6cm 0cm,clip=true,width=\textwidth]{figures/icassp2.png}
    \caption{The architecture of CLAR and GNNs. The orange lines denote CLAR components and the blue ones are GNNs.}
    \label{fig:clar}
\end{figure*}

\subsection{Sampling on the Complement}
The spectral character is hard to obtain directly from the complement, because the complement is greatly dense. To this end, we present two fast sampling strategies on the complement as below.

\textit{Node-based Sampling.}
For each node in $\mathcal{V}$, we sample a fixed number of edges $\mathcal{E}_{node} \subset \bar{\mathcal{E}}$ to construct the sampled graph $\mathcal{G}_{node}=\left(\mathcal{V},\mathcal{E}_{node}\right)$. $\mathcal{G}_{node}$ is a spanning subgraph of the complement $\bar{\mathcal{G}}$. Specifically, given a base number of sampling $S$, for each node $u \in \mathcal{V}$, we sample $S$ nodes $
\{u_1,u_2,u_3,\cdots,u_S\}$ without replacement, if and only if $\left(u,u_i\right) \in \bar{\mathcal{E}}$ where $i=1,2,3,\cdots,S$.
 
\textit{Edge-based Sampling.}
Besides, we further consider the influence of node degrees. This is based on the idea that if a node is connected to more nodes, whose distinction can be more easily erased by relatively dense lower-order information. At this time, the higher-order information should be introduced more. Node degrees are fully expressed in $\mathcal{E}$. In specific, we firstly take the head nodes of every edges that $\mathcal{V}_{head} = \left(v_i,i=1,2,3,\cdots,|\mathcal{E}|\right)$, where $\mathcal{E} = \{\left(v_i, v_j\right)\}$. Then we sample the tail nodes $\mathcal{V}_{tail} = \left(\bar{v}_j, \bar{v}_j \in \mathcal{V}\right)$, if and only if $\exists v_i \in \mathcal{V}_{head}, \left(v_i, \bar{v}_j\right) \in \bar{\mathcal{E}}$. Here, $|\mathcal{V}_{head}|$ and $|\mathcal{V}_{tail}|$ are not restricted to be the same. Similar to $S$ in node based sampling, we introduce $S$ to repeat $\mathcal{V}_{head}$ as $S$ times to meet $|\mathcal{V}_{tail}|$. Finally, by a pairing combination of $\mathcal{V}_{head}$ and $\mathcal{V}_{tail}$, we get $\mathcal{E}_{edge}$, and $\mathcal{G}_{edge} = \left(\mathcal{V}, \mathcal{E}_{edge}\right)$ as the sampled graph.

To be simplified, we uniform the sampled graph obtained via the different methods as  $\mathcal{G}_{s}=(\mathcal{V}_{s},\mathcal{E}_{s})$. Please refer to  Algorithm~\ref{alg:sample} in Appendix~\ref{app:sampling} for the sampling strategy $\mathtt{SAMPLE}$.



\subsection{Complement Laplacian Regularization}
We follow the traditional graph-based semi-supervised node classification task to obtain CLAR. To start with, the objective function is~\citep{kipf_deep_2020}, 
\begin{equation}
    \mathcal{L}=\mathcal{L}_{sup}+\gamma\mathcal{L}_{reg},
    \label{equ:semi}
\end{equation}
where $\mathcal{L}_{sup}$ is the supervised classification loss, and $\gamma$ is the weighting factor of the Laplacian regularizer $\mathcal{L}_{reg}$. This regularizer constrain the similarity of the connected nodes' representations (Eq~\ref{equ:reg}).
\begin{equation}
    \mathcal{L}_{reg}=\sum_{i,j}A_{ij}||f\left(x_i\right)-f\left(x_j\right)||^2
    =\tr\left(f\left(X\right)^TLf\left(X\right)\right).
    \label{equ:reg}
\end{equation}
To be clear, the topological similarity is totally captured by $\mathcal{L}_{reg}$, for $f\left(x\right)$ is a node-node-independent classifier.

However, the Laplacian regularization (i.e., $\mathcal{L}_{reg}$ in Eq. \ref{equ:semi}) is redundant on GNNs~\citep{DBLP:conf/aaai/0002MC21}, because GNNs (Eq.\ref{equ:gnn_layer}) covers this regularization \citep{kipf_deep_2020}, both are low-pass filters. We provide spectral analysis in Sec.~\ref{sec:math}.
%
In this paper, we instead construct Laplacian regularization on the extracted complement $\mathcal{G}_{s}$, building the high-pass filters from the negation of the low-pass ones of GNNs, that
\begin{equation}
    \mathcal{L}_{com}=\tr \left(f(X,A)^T\mathrm{L}(\tilde{A_s})f(X,A)\right),
    \label{equ:com}
\end{equation}
where $\tilde{A_s}$ is the adjacency matrix reduced on $\mathcal{G}_{s}$ with normalization. While $\mathtt{SAMPLE}$ is uncontrollable, we append the Laplacian regularization to balance the condition (i.e., Eq.~\ref{equ:ori}).
\begin{equation}
    \mathcal{L}_{ori}=\tr \left(f(X,A)^T \mathrm{L}(\tilde{A}) f(X,A)\right)
    \label{equ:ori}
\end{equation} 
Therefore, CLAR is composed of the two regularization components, with hyper-parameters $\alpha$ and $\beta$ to adjust.
\begin{equation}
    \mathcal{L}_{CLAR}=\alpha \mathcal{L}_{ori}+ \beta \mathcal{L}_{com},
\end{equation}
In general, the enhanced GNNs with CLAR supplementing high-pass filters can be achieved by the objective function:
\begin{equation}
    \mathcal{L} = \mathcal{L}_{cls} + \mathcal{L}_{CLAR}, 
\end{equation} 
where $\mathcal{L}_{cls}$ is the classification loss of GNNs (e.g., Eq.~\ref{equ:semi}).




